Learning Graph-Enhanced Commander-Executor for Multi-Agent Navigation

This paper investigates the multi-agent navigation problem, which requires multiple agents to reach the target goals in a limited time. Multi-agent reinforcement learning (MARL) has shown promising results for solving this issue. However, it is inefficient for MARL to directly explore the (nearly) optimal policy in the large search space, which is exacerbated as the agent number increases (e.g., 10+ agents) or the environment is more complex (e.g., 3D simulator). Goal-conditioned hierarchical reinforcement learning (HRL) provides a promising direction to tackle this challenge by introducing a hierarchical structure to decompose the search space, where the low-level policy predicts primitive actions in the guidance of the goals derived from the high-level policy. In this paper, we propose Multi-Agent Graph-Enhanced Commander-Executor (MAGE-X), a graph-based goal-conditioned hierarchical method for multi-agent navigation tasks. MAGE-X comprises a high-level Goal Commander and a low-level Action Executor. The Goal Commander predicts the probability distribution of goals and leverages them to assign each agent the most appropriate final target. The Action Executor utilizes graph neural networks (GNN) to construct a subgraph for each agent that only contains crucial partners to improve cooperation. Additionally, the Goal Encoder in the Action Executor captures the relationship between the agent and the designated goal to encourage the agent to reach the final target. The results show that MAGE-X outperforms the state-of-the-art MARL baselines with a 100% success rate with only 3 million training steps in multi-agent particle environments (MPE) with 50 agents, and at least a 12% higher success rate and 2x higher data efficiency in a more complicated quadrotor 3D navigation task.

==> AAMAS-2023 Formatting Instructions/0_abstract.tex <==
\begin{abstract}
%现在有multi-agent navigation marl这个任务，然后marl有potential解决这个事情，但是他们都是直接底层执行action的，难以快速学明白自己想要干啥，训练效率低下，尤其是在大规模智能体的场景下，space 更大更难学。hrl这种分层的思想可以帮助解决这个事情。所以我们提出了xxxx。
This paper investigates the multi-agent navigation problem, which requires multiple agents to reach the target goals in a limited time. Multi-agent reinforcement learning~(MARL) has shown promising results for solving this issue. 
However, it is inefficient for MARL to directly explore the (nearly) optimal policy in the large search space, which is exacerbated as the agent number increases~(e.g., 10+ agents) or the environment is more complex~(e.g., 3$D$ simulator). 
Goal-conditioned hierarchical reinforcement learning~(HRL) provides a promising direction to tackle this challenge by introducing a hierarchical structure to decompose the search space, where the low-level policy predicts primitive actions in the guidance of the goals derived from the high-level policy. 
In this paper, we propose \emph{\underline{M}ulti-\underline{A}gent \underline{G}raph-\underline{E}nhanced Commander-E\underline{X}ecutor}~({\name}), a graph-based goal-conditioned hierarchical method for multi-agent navigation tasks. {\name} comprises a high-level \emph{Goal Commander} and a low-level \emph{Action Executor}. The \emph{Goal Commander} predicts the probability distribution of the goals and leverages them to assign the most appropriate final target to each agent. 
The \emph{Action Executor} utilizes graph neural networks~(GNN) to construct a subgraph for each agent that only contains its crucial partners to improve cooperation. Additionally, the Goal Encoder in the \emph{Action Executor} captures the relationship between the agent and the designated goal to encourage the agent to reach the final target.
The results show that {\name} outperforms the state-of-the-art MARL baselines with a 100\% success rate with only 3 million training steps in multi-agent particle environments~(MPE) with 50 agents, and at least a 12\% higher success rate and 2$\times$ higher data efficiency in a more complicated quadrotor 3$D$ navigation task. 

% As a result, the existing methods mainly focus on the navigation task with few agents in the simple simulator.


% We tackle the problem of multi-agent navigation which is a complex and long-horizon task suffering from large observation and action spaces. Goal-conditioned Multi-agent Reinforcement Learning~(MARL) offers the solution to this problem via task decomposition. However, it is confronted with the inefficiency of sub-goal assignment and unsatisfying cooperation in low-level action execution, especially in scenarios with a large number of agents. In this paper, we propose \emph{\underline{M}ulti-\underline{A}gent \underline{G}raph-enhanced Command\underline{e}r-Executo\underline{r}}~({\name}), a graph-based goal-conditioned method for multi-agent navigation tasks. The high-level Goal Commander leverages the probability prediction of goals to assign each agent the most appropriate final target. The low-level Action Executor utilizes graph neural networks~(GNN) to construct a subgraph for each agent that only contains crucial partners to improve cooperation. Additionally, the Goal Encoder in the Action Executor captures the relationship between the agent and the designated goal to encourage the agent to reach the final target. The State Extractor endows the team representation in the subgraph with strong goal guidance.
% The results show that {\name} converges much faster and outperforms the state-of-the-art MARL baselines {\bf by a large margin} in multi-agent particle environments~(MPE) with a massive number of agents and a more complicated quadrotor navigation task.







% gym-pybullet-drones.

%多智能体导航需要快速到达指定目标点，他是一个长序列决策问题上存在动作空间大的问题，特别大规模上，观测空间也巨大，使得策略很难去优化。goal-coditioned marl提供了一个解决思路，他将长序列问题分解，使搜索空间降维，但是还存在goal分配将空间分离的低效性。为了解决多机大观测空间和动作空间，我们将gnn和hmarl相结合，提出了mager，一种graph-enhanced commander-executor，首先在commander层级利用reward 驱动去为每个智能体分配最佳的目标点。在executor层级利用gnn为每个智能体裁剪子图，只关注对自己有效的partners。我们在粒子环境中的大规模智能体导航和推球任务以及偏物理仿真的无人机环境中，和现有sota的marl baselines中进行对比，都达到了sota的性能。

\end{abstract}

%%% The code below was generated by the tool at http://dl.acm.org/ccs.cfm.
%%% Please replace this example with code app【】ropriate for your own paper.


%%% Use this command to specify a few keywords describing your work.
%%% Keywords should be separated by commas.

\keywords{Multi-agent Reinforcement Learning, Goal-conditioned Reinforcement Learning, Multi-agent Navigation, Graph Neural Network}

==> AAMAS-2023 Formatting Instructions/1_intro.tex <==

\section{Introduction}
%navigation是目前机器人的一个典型任务，在自动驾驶、物流配送、抢险救灾等领域广泛使用。单智能体导航存在长序列决策动作空间巨大的问题，再拓展至大规模多智能体多目标点导航上，还存在任务分配和观测空间大的问题，导致很难达到最优解。drl的出现提供了解决方案，drl可以利用自动训练网络去优化拟合复杂多变的策略.
% 第一段 第二段multi agent navigation这个事情,multi-agent in marl这个事情，3讲效率，4 引入hrl和gnn，5 我们
Navigation is a typical task in the intelligent agent system, applied in a wide range of applications, such as autonomous driving~\cite{autonomousdriving,autonomousdriving2}, logistics and transportation~\cite{logistics,logistics2}, and search and rescue for disasters~\cite{rescue,rescue2}. In this paper, we consider a multi-agent navigation task where multiple agents simultaneously move to the target goals in a cooperative fashion. Multi-agent reinforcement learning~(MARL) has attracted significant attention due to its powerful expressiveness in multi-agent navigation tasks~\cite{maans,multinavigation, multi-navigation, inferenceMultiNavigation}.

The common approach to searching for the near-optimal solution in MARL~\cite{mappo,mat} is to directly train a policy that produces environmental actions for agents. However, learning the strategy directly from large search space results in low data efficiency, which is more severe as the number of agents or the complexity of the environment increases. Therefore, the existing methods in navigation tasks target simple scenarios with few agents.
Goal-conditioned HRL~\cite{gchrl_1,gchrl_2,gchrl_3,gchrl_4,gchrl_5,gchrl_6,gchrl_7} has been recognized as an effective paradigm to address this problem, comprising a high-level policy that breaks the original task into a series of subgoals and a low-level policy that aims at the arrival of these subgoals. Recent works~\cite{maser,LGA} in goal-conditioned HRL mainly focus on developing high-level policies for providing agents with appropriate subgoals. However, designating the subgoals may confuse agents on which target goals they should reach.

% , recent works~\cite{maser,gchmarl_2,gchmarl_3} extend single-agent methods to multi-agent environments without considering the cooperation among agents in large observation and action spaces. As a result, they are not applicable in multi-agent navigation tasks, especially in scenarios with a massive number of agents.

%现有的drl方法在单机导航任务上有人提出goal-conditional hrl的方法，分开了两层策略，通过上层通过reply buffer里面的状态，输出subgoal，下层输出action，将动作空间降维，加快了训练效率[1][2][3]。也有到多机导航上，但是只是做了简单的扩展[4]。然而这种对于大规模智能体来说，未考虑到任务分配调度和多目标点，并不能很好的拓展至多智能体导航任务上。
Graph neural networks~(GNN) have been widely applied in multi-agent cooperative tasks due to their effective learning of agents' graph representations. The literature on GNN~\cite{MAGIC,DICG,gnn_3} in MARL constructs a graph whose nodes represent agents' information to model the interaction among them and encourage agents to cooperate. To enhance the cooperation among agents, we can leverage GNN in the low-level policy in HRL to capture the relationship of agents and express preferences for different teammates.


% with additional information of goals.  

%而在大规模任务上，为了解决观测空间大的问题，提高合作性，有人用transformer[6]或者gnn[7]去建模智能体之间的关系，提高合作性。但是这带来的问题在于她只考虑了agent之间的关系，target goal并没有考虑进来，如果单纯在goal放进来会增加维度。难以训练。

To improve data efficiency and cooperation, we propose \emph{\underline{M}ulti-\underline{A}gent \underline{G}raph-\underline{E}nhanced Commander-E\underline{X}ecutor}~({\name}), a graph-based goal-conditioned hierarchical framework in multi-agent navigation tasks. {\name} consists of two components, the high-level {\bf Goal Commander} and the low-level {\bf Action Executor}. For the target-goal assignment, the {\bf Goal Commander} infers the probability distribution of target goals to assign the most appropriate target goal for each agent instead of the subgoal.
% based on which each agent is assigned the most appropriate target goal. 
As a result, the multi-agent navigation is converted to multiple single-agent navigation tasks in the multi-agent environment, in which each agent is required to reach the designated goal while avoiding collisions.
% with little collision. 
In the {\bf Action Executor}, we take advantage of GNN to perceive the relationship among agents and produce a subgraph for each agent to decide to whom they should pay attention.
% to pay attention.
After that, the State Extractor receives the correlation between the agent and its target goal from the Goal Encoder and the agent's embedded feature in the subgraph to empower the team representation with strong goal guidance, promoting agents to reach target goals. The suggested scheme is challenged against MARL baselines in multi-agent particle environments~(MPE)~\cite{mpe} with a massive number of agents and a more complicated quadrotor navigation task~\cite{drone}. The experimental results demonstrate that {\name} outperforms the MARL baselines, achieving a 100\% success rate with only 3 million training steps in MPE with 50 agents. Furthermore, {\name} attains at least a 12\% higher success rate and 2$\times$ higher data efficiency in the quadrotor navigation task.
% x2 

Our contributions can be summarized as follows:
\setlength{\parskip}{0pt} 
\setlength{\itemsep}{0pt plus 1pt}
\begin{itemize}
\item We introduce a graph-based goal-conditioned framework in multi-agent navigation tasks, \emph{Multi-Agent Graph-enhanced Commander-Executor}~({\name}), to solve the problem of data efficiency and cooperation in large search space.
\item We develop a high-level Goal Commander, which utilizes the probability distribution of goals to allocate each agent to the most appropriate target goal.
\item We propose the low-level Action Executor, which adopts GNN to improve the coordination, and the Goal Encoder and the State Extractor to encourage agents to complete the task.
\item {\name} converges much faster and substantially outperforms MARL algorithms in multi-agent particle environments~(MPE)~\cite{mpe} with a massive number of agents and a quadrotor navigation task~\cite{drone}.
\end{itemize}
%针对以上问题，我们提出了基于graph增强的分层多目标多机导航方法。将任务进行分解，首先上层分配器利用专家指导奖励驱动的形式将多目标合理分配给每个智能体。下层执行器利用图神经网络建模智能体之间的关系，构成子图，降低了图的规模，再和目标点编码器输出下一步该执行的动作。通过实验证明，我们的方法在粒子环境和无人机环境下都实现了数据效率xx%的提升，性能有xx%的提升。


==> AAMAS-2023 Formatting Instructions/2_related.tex <==
\section{Related Work}
%navigation  MARL navigation 
%goal con   不足：多智能体只有简单地拓展，没有专门的设计（大动作空间 状态空间 分层降维），
%gnn  magic DICG  目前仅在agent之间构建graph 没有针对goal进行设计


% 
\subsection{Navigation}
Navigation has been widely investigated in recent years, where RL has shown its ability to solve various applications~\cite{navigation1, navigation2, navigation3, save}. For example, Rao~\cite{visualnavigation} presents a model-embedded actor-critic architecture for the multi-goal visual navigation task. This embedded model consists of two auxiliary task modules, a path closed-loop detection module to understand whether the state is experienced and a state-target matching module to distinguish the difference between states and goals. Furthermore, Zhu~\cite{navigation1} introduces a target-driven actor-critic model to achieve greater adaptability and flexibility for the target-driven visual navigation task.

As for multi-agent navigation tasks in MARL~\cite{multinavigation, multi-navigation, inferenceMultiNavigation,maans}, the difficulties lie in data efficiency and cooperation in large space spaces, which is exacerbated as agent number increases and the environment becomes more complicated. EPS~\cite{multi-navigation} is introduced to enhance exploration efficiency and improve sample efficiency in multi-robot mapless navigation, which uses the evolutionary population periodically generated from robots’ policies to search for different and novel states. Furthermore, Xia~\cite{inferenceMultiNavigation} proposes an inference-based hierarchical reinforcement learning framework~(IHRL) to address the multi-agent cooperative navigation problem via the interplay of high-level inference and low-level actions. The proposed {\name} specializes in navigation tasks and outperforms the MARL baselines with high sample efficiency.

%Hu~\cite{sim2real} proposes a novel sim-to-real pipeline with a deep reinforcement learning architecture to help the agent navigate efficiently to the target in rough real-world 3D terrain environments. In this pipeline, several policies are trained in the simulation for addressing different reality gaps. 

\subsection{Goal-conditioned HRL}
Goal-conditioned hierarchical reinforcement Learning~(HRL) has shown its capability in a wide range of tasks~\cite{goalconditioned1,HForesight,goalhierarchical} with a hierarchy consisting of high-level and low-level policies. The high-level policy generates intermediate subgoals every global timestep, which is regarded as a goal guidance of the low-level policy. 

Kreidieh~\cite{multiHRLgoal} addresses the challenges of the interactions between high-level and low-level agents by introducing inter-level cooperation. This inter-level cooperation is given by modifying the high-level policy's objective function and subsequent gradients. 
Another representative is LGA~\cite{LGA}, where the subgoal assignment is parameterized as latent variables to be trained. LGA directly provides primitive actions for agents depending on latent variables to accomplish multi-agent tasks. 
MASER~\cite{maser} automatically produces subgoals for agents from the experience replay buffer relying on both individual and total Q-values. Besides, it adopts the individual intrinsic reward for each agent to reach the assigned subgoals and maximize the joint action value. 
However, the generation of subgoals may be inefficient since the correspondence between subgoals and the final goals is implicit. In this paper, {\name} utilizes the goal-conditioned hierarchical framework in multi-agent navigation tasks to improve the sample efficiency, where the high-level policy deals with target-goal assignment and the low-level policy deals with the action execution for each agent.

\subsection{Graph Neural Networks}
Graph neural networks~(GNN)~\cite{gnn} are broadly used due to their effective learning of graph representations and the ability to capture the relationships of different graphs. Recently, several works have applied GNN in multi-agent systems to model agents' interactions. HAMA~\cite{gnn_hierarchical} proposes a hierarchical graph attention network that captures the underlying relationships at the agent-level and the group-level, enhancing generalization and scalability. MAGIC~\cite{MAGIC} is a novel graph communication protocol that implies the topology of agents' interactions, helping agents decide when to communicate and with whom to communicate. DICG~\cite{DICG} leverages dynamic coordination graphs to infer joint actions and values implicitly. GCS~\cite{GCS} learns coordinated behaviors by factorizing the joint team policy into a graph generator and a graph-based coordinated policy. The generator captures the underlying dynamic correlation of agents, which is then exploited by the graph-based coordinated policy. The Action Executor of {\name} benefits from GNN to capture the team representation and introduces a Goal Encoder and a State Extractor to strengthen the expression of target goals.


==> AAMAS-2023 Formatting Instructions/3_preliminary.tex <==
\section{Preliminary}
%dmdp 
%gnn

\begin{figure*}[t!]
	\centering
    \includegraphics[width=1.0\linewidth]{AAMAS-2023 Formatting Instructions/figures/framework.png}
	\centering \caption{{Overview of \emph{Multi-Agent Graph-enhanced Commander-Executor}}  (\name).}
\label{fig:Framework}
\end{figure*}
\subsection{Dec-MDPs}
In this paper, we consider a variant of MDP to solve the decentralized control problem in stochastic environments called Decentralized Markov Decision Processes~(Dec-MDPs).

Here, the multi-agent Dec-MDPs problem is formulated as:
\begin{equation}
<\mathcal{N},\mathcal{S}, \mathcal{A}, \mathcal{T}, R, G, \mathcal{O},\gamma>,
\end{equation}
where $\mathcal{N}\equiv\{1,...,n\}$ is a set of $N=|\mathcal{N}|$ agents. Note that $\mathcal{S}$ is a set of global states in the assumption that $\mathcal{S}$ is jointly observable. 
$\mathcal{A}$ is the action space of each agent, and $\mathbf{A}\equiv \mathcal{A}^N$ is the joint action space. $\mathcal{O}$ is the observation space. $R$ represents the reward function, and 
$R(s, \mathbf{a}, s')$ is the reward obtained from the transition of joint actions $\mathbf{a}\in\mathbf{A}$ from the state $s\in\mathcal{S}$ to the state $s^{\prime}\in\mathcal{S}$. $\gamma \in [0, 1)$ is the discount factor. $\mathcal{T}(s,\mathbf{a},s'):\mathcal{S}\times\mathbf{A}\times \mathcal{S}\mapsto [0,1]$ is the dynamics function denoting the transition probability. 
$G$ is the observation function, and $G(s, \mathbf{a}, s^{\prime}, o_i)$ is the probability of agents $i\in\mathcal{N}$ seeing observation $o_i\in\mathcal{O}$. 
% The discount return is $G_t = \sum^{\inf}_{l=0}\gamma^{l} r_{t+l}$, where $r_t$ is the joint reward at step $t$. 
Each agent has a policy $\pi^i(a^i_t|o^i_{1:t})$ to produce action $a^i_t$ from observations $o^i_{t}$ at step $t$. And agents need to maximize the expected discounted return $\mathbb{E} \sum^{\inf}_{l=0}\gamma^{l} r_{t+l}$, where $r_t=R(s_{t}, \mathbf{a}_t, s_{t+1})$ is the joint reward at step $t$.


% We figure out some important inferences. A 2-agent DEC-MDP is a DEC-MDP such that the world state can be factored into two components, $S = S_1 \times S_2$. This 2-agent DEC-MDP is said to be locally fully observable if $ \exists o_i$ ,$\forall s_i : P(s_i|o_i)=1$. It is recognized to be reward independent,  $R((s_1,s_2),(a_1,a_2),(s^{\prime}_1,s^{\prime}_2)) = R_1(s_1, a_1, s^{\prime}_1)+R_2(s_2,a_2,s^{\prime}_2)$ if $R_1$ and $R_2$ exist.

\subsection{Graph Neural Networks}
Graph neural networks~(GNN) are a special type of neural network capable of dealing with data in the graph structure. The critical ingredient of GNN is pairwise message passing, i.e., graph nodes iteratively update their representations by exchanging information with their neighbors. The general formula is given as below:

\begin{equation}
    h_i^{(l)} = \sigma ( \sum_{j\in N_i} \frac{1}{\sqrt{d_i d_j}}(h_j^{l-1}W^{(l)}) ),
    \label{eq:GNN}
\end{equation}
where $h_i$ is the feature vector of node $i$. $N_i$ represents a set of neighbouring nodes of $i$ and $W^{(l)}$ is the learnable weights in the layer $l$. $\sigma$ is the activation function. $d_i$ is the dimension of feature stored in node $i$. Equation~\ref{eq:GNN} shows that the feature of node $i$ will be influenced by its neighbors. In this paper, we use graph convolutional networks~(GCN)~\cite{gcn} to model the interaction of agents. GCN is a variant of convolution neural networks~(CNN) to be applied in the data with graph structure.


==> AAMAS-2023 Formatting Instructions/4_method.tex <==
\section{Methodology}


\begin{figure*}[t!]
	\centering
    \includegraphics[width=0.95\linewidth]{AAMAS-2023 Formatting Instructions/figures/architecture.png}
	\centering \caption{Workflow of Action Executor, including a Subgraph Extractor, a Goal Encoder, a State Extractor for representation learning and an Action Generator.}
\label{fig:architecture}
\end{figure*}
In this section, we introduce the proposed framework, {\name}, to improve sample efficiency and the cooperation in multi-agent navigation tasks. The overview of our framework is demonstrated in ~\cref{fig:Framework}. {\name} comprises two components, the Goal Commander and the Action Executor. The high-level Goal Commander follows the principles of centralized-training-centralized-execution (CTCE). In contrast, the low-level Action Executor is in a decentralized setting with partial observation of $N$ agents, where agent $k$ receives local observation, $o_{t}^k$, at step $t$. Agent $k$ learns the policy, $\pi_k$, to produce a distribution over actions at each time step $t$, $a_{t}^k\sim\pi_{k}(a_{t}^k|o_{t}^k)$. The process of a navigation task begins with the Goal Scheduler in the Goal Commander receiving the spawn locations of all the agents and the target goals. The probability distribution of the target goals is predicted by the scheduler, and each agent is assigned the most appropriate target goal rather than the subgoal. Therefore, the multi-agent navigation is converted to multiple single-agent navigation tasks in the multi-agent environment, where each agent is required to reach the given goal as quickly as possible while avoiding collisions. Take agent $k$ as an example. The Subgraph Extractor takes in the observation of agent $k$ and other agents and produces the subgraph of agent $k$ only including its crucial neighbors to improve cooperation. The relationship of agent $k$ and its target goal is extracted from the Goal Encoder, which is then sent to the State Extractor combined with the feature of agent $k$ in the subgraph to endow the team representation with strong goal guidance. Finally, agent $k$ takes the preliminary action from the Action Generator to complete the navigation task. 
%framework介绍:为了解决大状态空间，大动作空间的问题，我们提出了mager，考虑partial observation的情况，上层centralized，下次decentrailized，每个agent输出自己的action。figure 1展示了我们的framework，首先是在unseen-map上生成agengs和目标点，将他们的xy位置输出给上层的goal commander里的goal scheduler，scheduler根据所有agent和goal的状态，进行一一分配。分配好的agent和目标点相当于是将联合任务分解为了单体任务，到了下层agent只需要在避免碰撞的情况下，最快到达目标点。下层executor是分布式的结构，他先拿到所有agent的信息，进入subgrpah extractor，然后输出对当前agentk的subgraph。对于agentk的target goal，我们把它放进goal encoder 提取feature，最后将goal feature和subgraph里面agentk的node k的feature 进行融合，输入state extractor得到最终关于agent与agent之间，agent与goal之间的映射，输出priminary action执行动作。
% However, reinforcement learning has the potential to figure out the near optimal and feasible solution via automatic exploration and exploitation. 
\subsection{Goal Commander}
Goal assignment is a long-studied maximal matching problem, especially in scenarios with large-scale agents. The Goal Commander builds upon a Goal Scheduler module for target-goal assignment, which produces the probability distribution of target goals. The designed reward is related to the distance cost of the Hungarian algorithm~\cite{Hungarian}, a state-of-the-art classical method to tackle the combinatorial optimization algorithm in graph theory.   
%high level：assignment方法 reward design。目前多目标点分配问题还存在很大的问题，NP hard 问题，我们只能找到近似最优解。我们运用了匈牙利算法作为专家指导，去计算我们的reward，通过输出的goal的概率分布去为每个agent分配目标点。

\textbf{Goal Scheduler}: This module is made up by a Multi-Layer Perception~(MLP) layer, $f_{sche}$, that takes the positions of all agents, $P_a$, and the positions of target goals, $P_g$, as input. We obtain the probability of the target goals, $P_{goal}$, by computing the softmax operator over the output of $f_{sche}$:
    \begin{equation}
    P_{goal} = Softmax(f_{sche}(P_a,P_g)).
    \end{equation}
Thereafter, $P_{goal}$ is ranked in decreasing order and the reordered goals $1...N$ are sequentially assigned to agent $1...N$. The reward of the Goal Scheduler, $R_{c}$, represents the distance cost of our assignment strategy, $C_{c}$, against the distance cost of the Hungarian algorithm, $C_{h}$:
    \begin{equation}
    R_{c} = 1-\frac{C_{c}}{C_{h}}.
    \end{equation}

%所有agent和target goal的X,Y（二维）或者xyz（三维）position作为输入进入goal scheduler。goal scheduler由多层mlp组成。给个公式。输出为每个点的softmax后的概率分布，再进行argmax排序，最大的分配给agent0，以此类推。其中我们用匈牙利算法计算出来的distance-cost作为一个专家指导作用于reward，得到一个相对的偏差，目标是你和匈牙利，甚至比他还要好，即reward=1-our cost/expert cost。给个公式。


\subsection{Action Executor}
The Action Executor is designed for high cooperation where agents speedily reach the designated goal with little collision in the multi-agent environment. The workflow of the Action Executor is illustrated in~\cref{fig:architecture}. It consists of the Subgraph Extractor, the Goal Encoder, the State Extractor, and the Action Generator. The Subgraph Extractor encodes the observations of all agents and yields a subgraph for agent $k$ only containing the crucial teammates. 
The Goal Encoder extracts the correlation of agent $k$ and its assigned goal, which is then fed into the State Extractor with the feature of agent $k$ in the subgraph to endow the team representation with target goal guidance. Finally, the Action Generator produces the action for the agent $k$. 

The environmental reward for each agent, $R_{e}$, is the linear combination of the complete bonus, $R_b$, the distance penalty, $R_d$, and the collision penalty, $R_c$:
 \begin{equation}
    R_{e} = \alpha{R_b}+\beta{R_d}+\gamma{R_c},
    \end{equation}
where $\alpha$, $\beta$ and $\gamma$ are the coefficient of $R_b$, $R_d$ and $R_c$, respectively.

%Action Executor是为了更好地增强智能体之间的合作性，使得智能体在多智能体环境中，可以更快地到达目标点，避免碰撞。如图所示，action executor 由xxx组成，首先subgraph extractor 会编码每个智能体的observation，输出subgraph，只包含重要智能体的编码信息。goal encoder编码agentk的target goal k，输出的东西和subgraph中当前智能体k的feature一同输入进state extractor去捕捉xx和xx之间的关系。最后action generator会输出action，执行动作。
%奖励是碰撞惩罚和agent到目标点的距离城府和到达目标点的奖励

\textbf{Subgraph Extractor: }The Subgraph Extractor is comprised of the Observation Encoder and the Graph Encoder. In the Observation Encoder, we apply an MLP layer $f_{o}$ to encode the observations of all agents and GCN to produce a fully connected graph of agents, $G_{a}$. This can be formulated as:
 \begin{equation}
G_a = GCN\left(\left(f_o(o^1),f_o(o^2),..f_o(o^N)\right),A_f\right),
    \end{equation}
where $A_f$ is denoted as an adjacent matrix of a fully connected graph. In the Graph Encoder, we compute the gumbel softmax~\cite{gumbel_softmax} over the feature of $G_{a}$ updated by an MLP layer, $f_{g}$. Thus, we can obtain an adjacent matrix of $A_s^k$ through it:
\begin{equation}
    A_s = Gumbel\_Softmax(f_g(G_a)).
    \end{equation}
    
Afterwards, we use GCN to generate $G_s^k$:
    \begin{equation}
    G_s^k = GCN(G_a,A_s^k).
    \end{equation}
The feature of the agent $k$ in $G_s^k$ is then sent to the State Extractor. Note that there are $l_{g}$ blocks in the Graph Encoder.
%subgraph extractor由两个encoder组成，首先在obs encoder，all agent observation 由mlp encoder，再经过gcn获得一个全连接的graph。然后进入graph encoder，这个全连接的graph经过mlp和gumbel softmax就输出一个子图link，和feature一起进入gcn，note that这个操作循环了nf次=2次。最后输出子图中self feature进入state extractor。

\textbf{Goal Encoder and State Extractor: }To capture the correlation between the agent $k$ and its assigned goal, the Goal Encoder comprises an MLP layer $f_{goal}$, and takes in the target goal's position $P_g^k$, and the agent's observation $o^k$. This can be formulated as:
\begin{equation}
    E_{goal}^{k} = f_{goal}(P_g^k,o^k).
    \end{equation}
    
Receiving the relationship between the agent and its target goal and the embedded feature of agent $k$ in $G_{s}$, $E_{a}^k$, we leverage the State Extractor to enhance the team representation with target goal guidance and output $E_{all}^k$. The State Extractor consists of an MLP layer $f_{state}$, and recurrent neural networks~(RNN) in consideration of the high correlation between current and historical states:
\begin{equation}
    E_{all}^k = RNN\left(f_{state}\left(concat\left(E_{goal}^k,E_{a}^k\right)\right)\right).
    \end{equation}
%lower level：graph enhanced方法 reward design
%Goal encoder是用来给target goal和current agent cincat起来进行一个特性提取的，就是用mlp layer输入target landmark的xy和current agent observation，然后输出的是agent和lankmark之间的关系。
%得到agent 和lankmark之间的关系后再与subgraph里面current agent的feature提取出来，此时的agent feature也融合了agent之间的关系，故他们concat起来过mlp。因为当前状态和历史状态的有关的，所以还使用了rnn去捕捉当前信息和历史信息的关系。
\subsection{Multi-agent Commander-Executor Training}

%training 公式 , observation of all agents $O$.

\begin{algorithm}
    \caption{Training Procedure of \emph{\name}}
    \label{algo:algo_mager}
    \begin{algorithmic}[1]
        \REQUIRE The positions $P_a$ of all agents, the joint observation $\mathbf{o}$ of all agents , and the positions $P_g$ of target goals.
        \ENSURE Final policy $\pi_\theta$ for the Goal Commander and $\pi_{\theta'}$ for the Action Executor.
        \STATE {\bf Initialize:} agents number $N$, maximal steps in an episode $T_e$, params in the Goal Commander $\theta$, $\phi$, params in the Action Executor $\theta'$, $\phi'$, the Goal Commander buffer $D$, the Action Executor buffer $D'$.
        \WHILE{$\theta$ and $\theta'$ not converges}
            \STATE{Reset environment and get $P_a$, $P_g$.}
            \STATE {\bf Initialize:} the step-count $t\leftarrow 1$ in $D$, the step-count $t'\leftarrow 1$ in $D'$.
            \STATE{ $P_{goal}\leftarrow$  \textbf{Goal\_Commander$(P_{a}$, $P_{g})$}.}
            \STATE{Calculate $\pi_\theta(a_t|\mathbf{o}_t)$ and $V_\phi(\mathbf{o}_t)$.}
            \STATE{Perform $a_{t}\sim\pi_\theta(a_t|\mathbf{o}_t)$.}
            \WHILE{$t'<T_e$ and not terminal}
                \STATE{$E_{all}^k\leftarrow$ \textbf{Action Executor ($\mathbf{o}$, $P_g^k$) } for each agent $k$}
                \STATE{Calculate $\pi_{\theta'}({a'^k_{t'}} |{o'^k_{t'}})$ and $V_{\phi'}({o'^k_{t'}})$ for each agent $k$.}
                \STATE{Perform $a'^k_{t'}\sim \pi_{\theta'}(a'^k_{t'} |{o'^k_{t'}} )$ for each agent $k$.}
                \STATE{Receive $r'_{t'}$ and ${o'^k_{t'+1}}$ for each agent $k$.} 
                \STATE{Store $({o'^k_{t'}},{a'^k_{t'}},\pi_{\theta'},({a'^k_{t'}}|o'_{t'}),V_{\phi'}({o'^k_{t'}}),r'_{t'},{o'}^k_{t'+1})$ in $D'$.}
                \STATE{$t'\leftarrow t'+1$}
            \ENDWHILE
            \STATE{Receive $r_t$ and $o_{t+1}$.}
            \STATE{$t\leftarrow t+1$}
            \STATE{Store $(o_t,a_t,\pi_\theta,(\mathbf{a}_t|\mathbf{o}_t),V_\phi(o_t),r_t,o_{t+1})$ in D.}
            \STATE{Perform update of $\theta$, $\phi$, $\theta'$ and $\phi'$.}
        \ENDWHILE
    \end{algorithmic}
\end{algorithm}


%我们有两个policy 网络，是去最大化reward和用的是mappo，其中一个上层的ctce网络，action space是所有goal的点的高斯分布和下层的ctde网，action space是智能体可行的离散动作。具体的算法如表1所示，
%The Goal Commander adopts the centralized decision setting, while the Action Executor observes the principles of centralized-training-decentralized-execution~(CTDE).
{\name}, following the goal-conditioned MARL framework, trains two policy networks for the Goal Commander and the Action Executor separately, which are optimized by maximizing the accumulated reward in the entire episode via reinforcement learning. We use Multi-agent Proximal Policy Optimization~(MAPPO)~\cite{mappo}, a multi-agent variant of Proximal Policy Optimization~(PPO)~\cite{ppo}, as the policy optimizer.

As shown in \cref{algo:algo_mager}, {\name} takes in the positions of agents, the observations of agents, and the positions of landmarks. Then, it produces the final policy $\pi_\theta$ for the Goal Commander and $\pi_{\theta'}$ for the Action Executor. First, we initialize the number of agents along with several training parameters, including maximal steps, parameters in the Goal Commander, parameters in the Action Executor, the Goal Commander reply buffer, $D$, and the Action Executor reply buffer, $D'$~(Line 1). 
The Goal Commander only performs one action every episode to assign the goals to agents in the beginning~(Line $5\sim7$) and receives the reward $r_t$ and the subsequent observation $o_{(t+1)}$ at the end of each episode, where $t$ represents the step-count in $D$~(Line 15 and 16). 
Thereafter, we update $\theta$ for the policy network $\pi_\theta$, and $\phi$ for the value network $V_{\phi}$, in the Goal Commander. 
Regarding the Action Executor, it outputs the action ${a'}^k_{t'}$ for each agent $k$, and stores a group of data in $D^{'}$ at each timestep $t'$~(Line $9\sim 13$). Similarly, we update $\theta'$ for the policy network $\pi_{\theta'}$, and $\phi'$ for the value network $V_{\phi'}$, in the Action Executor. \looseness=-1



% \begin{algorithm}
%     \caption{Training Goal Commander}
%     \label{algo:algo_gc}
%     \begin{algorithmic}[1]
%         \REQUIRE Position of all agents $P_a$ and target goals $P_g$
%         \ENSURE Selected target goals for all agents
%         \STATE Initialize max update M, agents N, thread L, max steps in an episode $T_e$, max steps in a batch $T_b$
%         \FOR{update = 1 to M, $d\theta \leftarrow 0$, $d\phi \leftarrow 0$}
%             \FOR{thread k = 1 to K}
%                 \STATE{Initialize params $\theta_{k}\leftarrow \theta$, $\phi_{k}\leftarrow \phi$, buffer D, step-count $t\leftarrow 1$}
%                 \WHILE{$t<T_b$}
%                     \STATE{Initialize thread step counter $t^{'}\leftarrow 1$}
%                     \STATE{Reset environment and get $P_a$,$P_g$}
%                     \STATE{$P_{goal} = Softmax(f_{sche}(P_a, P_g))$}
%                     \STATE{Calculate $\pi_{\theta_k}(\mathbf{a}_t|\mathbf{o}_t)$ and $V_{\phi k}(o_t)$}
%                     \STATE{Perform $a^{t}\sim\pi_{\theta_k}(\mathbf{a}_t|\mathbf{o}_t)$}
%                     \WHILE{$t^{'}<T_e$ and not terminal}
%                         \STATE{Perform step $9\sim 17$ in Algo.2 }
%                         \STATE{$t\leftarrow t+1$, $t^{'}\leftarrow t^{'}+1$}
%                     \ENDWHILE
%                     \STATE{Receive $r_t$ and $o_{t+1}$}
%                     \STATE{Store $(o_t,a_t,\pi_{\theta_k},(\mathbf{a}_t|\mathbf{o}_t),V_{\phi_k}(o_t),r_t,o_{t+1})$ in D}
%                 \ENDWHILE
%                 \STATE{Calculate $d\theta_k$ and $d\phi_k$ using D}
%             \ENDFOR
%             \FOR{thread $k = 1$ to $K$}
%                 \STATE{Accumulate gradients of $d\theta \leftarrow d\theta$  + $d_{\theta_k}$ and $d\phi \leftarrow d\phi$ + $d_{\phi_k}$}
%             \ENDFOR
%             \STATE{Perform update of $\theta$ using $d\theta$ and $\phi$ using $d\phi$}
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}
%     \caption{Training Action Executor}
%     \label{algo:algo_ae}
%     \begin{algorithmic}[1]
%         \REQUIRE The observation of all agents $O$ and assigned target goals $P_g$ 
%         \ENSURE Perform actions in the environment
%         \STATE Initialize max update $M^{'}$, agents $N$, thread $L$, max steps in an episode ${T_e}^{'}$, max steps in a batch ${T_b}^{'}$
%         \FOR{update = 1 to M, ${d\theta}^{'} \leftarrow 0$, ${d\phi}^{'} \leftarrow 0$}
%             \FOR{thread k = 1 to K}
%                 \STATE{Initialize params ${\theta_{k}}^{'}\leftarrow {\theta}^{'}$, ${\phi_{k}}^{'}\leftarrow {\phi}^{'}$, buffer $D^{'}$, step-count $t\leftarrow 1$}
%                 \WHILE{$t<{T_b}^{'}$}
%                     \STATE{Initialize thread step counter $t^{'}\leftarrow 1$}
%                     \STATE{Reset environment and get $O$,$P_g$}
%                     \WHILE{$t^{'}<T_e$ and not terminal}
%                         \STATE{$G_a = GCN((f_o(O_1),f_o(O_2),..f_o(O_N)),A_f)$}
%                         \STATE{$A_s = Gumbel\_Softmax(f_g(G_a))$}
%                         \STATE{${G_s}^{(i)} = GCN(G_a,{A_s}^{(i)})$ for each agent $i$}
%                         \STATE{$E_{goal}^{(i)} = f_{goal}({P_{g}}^{(i)},O^{(i)})$ for each agent $i$}
%                         \STATE{$E_{all}^{(i)} = RNN(f_{state}(concat(E_{goal}^{(i)},E_{a}^{(i)})))$ for each agent $i$}
                        
%                         \STATE{Calculate ${\pi^{'}}_{\theta_k}({{a^{'}}_i}^t|{{o^{'}}_i}^t)$ and ${V^{'}}_{\phi k}({{o^{'}}_i}^t)$ for each agent i}
%                         \STATE{Perform ${a^{'}}^{t}\sim{\pi^{'}}_{{\theta^{'}}_k}({{a^{'}}_i}^t|{{o^{'}}_i}^t)$ for each agent i}
%                         \STATE{Receive ${r^{'}}^t$ and ${{o^{'}}_i}^{t+1}$ for each agent i} 
%                         \STATE{Store $({{o^{'}}_i}^t,{{a^{'}}_i}^t,{{\pi}^{'}}_{{\theta^{'}}_k},({{a^{'}}_i}^t|{o^{'}}^t),{V^{'}}_{{\phi^{'}}_k}({{o^{'}}_i}^t),{r^{'}}^t,{{o^{'}}_i}^{t+1})$ in $D^{'}$}
%                         \STATE{$t\leftarrow t+1$, $t^{'}\leftarrow t^{'}+1$}
%                     \ENDWHILE
%                 \ENDWHILE
%                 \STATE{Calculate ${{d\theta}^{'}}_k$ and ${{d\phi}^{'}}_k$ using $D^{'}$}
%             \ENDFOR
%             \FOR{thread $k = 1$ to $K$}
%                 \STATE{Accumulate gradients of ${d\theta}^{'} \leftarrow {d\theta}^{'}$  + ${{d\theta}^{'}}_k$ and ${d\phi}^{'} \leftarrow {d\phi}^{'}$ + ${{d\phi}^{'}}_k$}
%             \ENDFOR
%             \STATE{Perform update of ${\theta}^{'}$ using ${d\theta}^{'}$ and ${\phi}^{'}$ using ${d\phi}^{'}$}
%         \ENDFOR
%     \end{algorithmic}
% \end{algorithm}

==> AAMAS-2023 Formatting Instructions/5_experiment.tex <==
\section{Experiments}

\subsection{Task Setup}
\label{sec:task_setup}
%为了验证我们算法的有效性，如图1所示，我们使用了三个任务simple spread 和push bal和drone在两个环境MPE和Pybullet-Gym-Drones里面进行了测试。其中simple spread 和push ball是common marl 环境with 5 20 50智能体，而Pybullet-Gym-Drones环境是更接近真实机器人环境的仿真器，他包含了飞机的动力学习模型，更加考验算法鲁棒性，需要更强飞机合作和到达目标点准确度。
To evaluate the effectiveness of our algorithm in large search space, we consider MPE~\cite{mpe} with a massive number of agents and pybullet-gym-drones~\cite{drone} in 3$D$ space as the experimental environments, as shown in Fig.~\ref{fig:env_mpe} and Fig.~\ref{fig:env_drone}. We select three typical tasks from these two environments: Simple Spread, Push Ball, and Drones. Then, we conduct experiments with $N\in\{5, 20, 50\}$ agents in Simple Spread and $N\in\{5, 20\}$ agents in Push Ball in MPE. 
Drone is a more complicated quadrotor navigation task in gym-pybullet-drones, which adopts aerodynamic models of quadrotors to narrow the gap between the simulation and the real world. Therefore, quadrotors in Drone require stronger cooperation to avoid the crash. We conduct experiments with 2 and 4 quadrotors in this 3$D$ simulator. 

\subsubsection{Simple Spread}
%simple spread 环境是一个2D典型的导航任务,他初始化N agent和N landmark，任务成功的标识为在有限时间步下，需要所有智能体到达全部目标地。智能体之间存在碰撞，碰撞会导致智能体互相弹开，影响状态和行走，我们reward的设计有distance penalty和success reward和碰撞的惩罚。智能体的动作空间为离散的上下左右，任务的难度随着智能体数量和空间范围扩大而增加。我们5agent是在2meter的空间中随机生成，20和50agent是分别在12m和20m的空间中按照图中b的四种地图形式生成的。目的是因为20和50agent十分密集，这四种map更加具有挑战性。实验证明，我们的算法具有更好的性能。

We utilize Simple Spread environment in MPE~\cite{mpe}, a classical 2D navigation task. The episode starts with the initialization of $N$ agents and $N$ landmarks. When all the agents reach the landmarks, this task is 100\% successful. The consequence of the collision between agents is that they will bounce off each other, which is detrimental to navigation efficiency. The available discrete actions of agents include \emph{Up}, \emph{Down}, \emph{Left}, and \emph{Right}. The task's difficulty increases with a larger agent number and map space. The experiment is conducted on 5, 20, and 50 agents. 
In the 5-agent setting, the spawn locations of agents and landmarks are random on the map with a size of 4. 
In the setting of $N\in\{20, 50\}$, the spawn locations of agents and landmarks are randomly initialized in four challenging maps with the size of 36 and 100, respectively, as shown in Fig~\ref{fig:env_mpe}(b). The horizons of steps in $N=5$, $20$, $50$ are 60, 100, and 120, respectively. 
%加上给60步，和100步和120步
%As the number of agents and the size of map become larger, random initialization of agents and landmarks may cause a vast variance of the arrangement of spawn locations, resulting in huge difference between final performances which is harmful to training. 
\begin{figure*}[ht!]
\captionsetup{justification=centering}
	\centering
    \subfigure[Simple Spread]
	{\centering
        {\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread.png}
    	}
    }
    \subfigure[Simple Spread with 20, 50 agents]
	{\centering
         {\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread_map1.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread_map2.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread_map3.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread_map4.png}
    	}
    }
    \subfigure[Push Ball]
	{\centering
        {\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball.png}
    	}
    }
    \subfigure[Push Ball with 20 agents]
	{\centering
        {\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball_map1.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball_map2.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball_map3.png}
    	}
    	{\includegraphics[height=0.18\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball_map4.png}
    	}
    }
	\caption{\raggedright{Experimental environments of Simple Spread and Push Ball in MPE. We remark that (b) represents simplified demonstration of 4 challenging task modes in Simple Spread, where the spawn locations of agents and landmarks are randomly distributed in the orange lines and the blue lines, respectively. (d) expresses simplified demonstration of 4 typical task modes in Push Ball, where the spawn locations of agents and landmarks are randomly distributed in the orange lines, and the spawn locations of balls are randomly distributed in the pink lines.}}
\label{fig:env_mpe}
\end{figure*}

\begin{figure}[ht!]
\captionsetup{justification=centering}
	\centering
    \subfigure
	{\centering
        {\includegraphics[height=0.25\textwidth]{AAMAS-2023 Formatting Instructions/figures/drone.png}}
    }
	\caption{Experiment environments of Drone.}
\vspace{-6mm}
\label{fig:env_drone}
\end{figure}

\subsubsection{Push Ball}
%Push ball 比simple spread任务难度进一步加大，他可以被认为是二阶段的导航任务，即需要智能体先找到小球，再attch住小球，去找到landmark，将小球投入landmark。故，他初始化N agent，N ball和N landmark，任务成功的标识为在有限时间步下，需要所有智能体带着小球到达全部目标地。与simple spread类似，不同在于，我们reward的设计有distance penalty和找到小球的success reward和到达landmark的success reward和碰撞的惩罚。我们5agent是在4meter的空间中随机生成，20agent是在16m的空间中按照图中d的四种地图形式生成的。目的是因为20agent十分密集，这四种map更加具有挑战性。实验证明，我们的算法具有更好的性能。
Push Ball is a more complicated two-stage navigation task in MPE~\cite{mpe}, requiring each agent to find the ball first, then push it into the landmark. At the beginning of each episode, $N$ agents, $N$ balls, and $N$ landmarks are initialized in the environment. The success rate of the task is the number of agents reaching the landmarks with the balls to the total number of all agents. The available discrete actions of agents include \emph{Up}, \emph{Down}, \emph{Left}, and \emph{Right}.
We conduct the experiments in the setting of 5 and 20 agents. In the scenarios of $N=5$, the spawn locations of agents, balls, and landmarks are randomly distributed on the map of size 16. For $N=20$, their initialization follows four challenging space arrangements on the map with a size of 144, as displayed in Fig~\ref{fig:env_mpe}(d). The horizons of the steps in $N=5$ and $20$ are 100 and 200, respectively. 
%加上给100步，和200步

\subsubsection{Drone}
%Drones 环境是基于pybullet的一个无人机3d仿真环境，支持导航任务。无人机对动力学模型进行建模，存在碰撞坠机等现实条件约束,他初始化N agent和N landmark，任务成功的标识为在有限时间步下，需要所有智能体到达全部目标地。智能体之间存在碰撞，碰撞会导致智能体坠机，任务失败，我们reward的设计有distance penalty和success reward和碰撞的惩罚。智能体的动作空间为离散的加速度xyz的方向。我们测试了2agent和4agent在空间中随机生成导航的实验。实验证明，我们的算法具有更好的性能。
We further adopt Drone in pybullet-gym-drones~\cite{drone}, a 3D simulator for flying quadrotors based on pybullet. Drone models the dynamics of quadrotors and controls them by adjusting the torque. Unlike MPE, the collision between quadrotors will lead to a crash and the failure of the task. In our navigation task, the spawn locations of $N$ quadrotors and $N$ landmark are random in the coordinates $x$ and $y$, but fixed in the coordinate $z$, with $x\in(-1.5,1.5), y\in(-1.5,1.5)$ and $z=1.5$. The task's objective is that quadrotors are required to reach all the landmarks on a limited time budget. The action space of each quadrotor is the direction of the acceleration in $x$, $y$, $z$ coordinate, containing \emph{Forward}, \emph{Backward}, and \emph{Stop} in each coordinate. We consider the experiments with $2$ and $4$ quadrotors. In our setting, the frequency at which the physics engine steps is 120 $HZ$; the max speed is 2 $m/s$, and the acceleration is 5 $m/{s}^2$. In every low-level step, we utilize the predicted acceleration direction to calculate each quadrotor's target velocity, and then the quadrotor executes the action every four physics engine steps. The horizon of the steps in $N=2$ and $4$ is 120. 
 
%加上我们设的是飞机动120hz每秒，每次走4秒，一共480步，每个action执行4步，执行120个action。我们设加速度为5m/s,限制的最大速度为2m/s，我们只输出加速度的方向然后根据加速度大小和方向和目前的速度去计算下一步的目标速度大小和方向赋值给controller。
\subsection{Implementation Details}
Each RL training is performed over 3 random seeds for a fair comparison. Each evaluation score is expressed in the format of "mean (standard deviation)", which is averaged over a total of 300 testing episodes, i.e., 100 episodes per random seed. In addition, we use the success rate, the number of landmarks reached by the agents to the total number of landmarks, to express the performance of each algorithm. In the Drone, we additionally consider the collision rate, the number of crashed quadrotors to the total number of quadrotors, to express the capability of cooperation. Our experimental platform involves a 128-core CPU, 256GB RAM, and an NVIDIA GeForce RTX 3090Ti with 24GB VRAM.
\begin{figure*}[ht!]
\captionsetup{justification=centering}
	\centering

        {\includegraphics[height=0.26\textwidth]{AAMAS-2023 Formatting Instructions/figures/simple_spread_all.png}
    	}

	\caption{\centering{Comparison between {\name} and other baselines in Simple Spread with $N=5$, $20$, $50$.}}
\label{fig:baseline_sp}
\vspace{-2mm}
\end{figure*}
\begin{figure}[ht!]
\captionsetup{justification=centering}
	\centering
    {\includegraphics[height=0.24\textwidth]{AAMAS-2023 Formatting Instructions/figures/push_ball_all.png}
    }

	\caption{\raggedright{Comparison between {\name} and other baselines in Push Ball with $N=5$, $20$.}}

\label{fig:baseline_pb}
\end{figure}
\begin{figure}[ht!]
\captionsetup{justification=centering}
	\centering     {\includegraphics[height=0.26\textwidth]{AAMAS-2023 Formatting Instructions/figures/drone_2_4.png}}
	\caption{\raggedright{Evaluation performance of the success rate and the collision rate between {\name} and baselines in Drone. The node in the upper left corner of the figure represents higher performance.}}
\vspace{-5mm}
\label{fig:drone_inter}
\end{figure}

\begin{figure*}[ht!]
\captionsetup{justification=centering}
	\centering
    
    {\includegraphics[height=0.26\textwidth]{AAMAS-2023 Formatting Instructions/figures/drone_collision_success_rate_baseline.png}}
     
\vspace{-3mm}
	\caption{\centering{Comparison between {\name} and other baselines in Drone.}}
\label{fig:baseline_drone}

\end{figure*}

\subsection{Baselines}
To demonstrate the effectiveness of our methods, we challenge it against four MARL baseline approaches.
\begin{itemize}
\setlength{\parskip}{0pt} 
\setlength{\itemsep}{0pt plus 1pt}
\item MAPPO~\cite{mappo}: This is the first and the most direct approach for applying PPO in MARL. It equips all agents with one shared set of parameters and updates the shared policy through agents’ aggregated trajectories.
\item Multi-Agent-Transformer~(MAT)~\cite{mat}: This is an encoder-decoder architecture that leverages the multi-agent advantage decomposition theorem to transform the joint policy search problem into a sequential decision-making process.
\item DICG~\cite{DICG}: This graph-based method comprises a module that infers the dynamic coordination graph structure and a GNN module that implicitly reasons about the joint actions or value based on the former module's output.
\item Maser~\cite{maser}: This is a goal-conditioned MARL method that automatically generates subgoals for multiple agents from the experience replay buffer by considering both the individual Q-value and the total Q-value.
\end{itemize}
\subsection{Main Results}
We present and analyze the experiment results of {\name} and MARL baselines in three competitive environments.

\subsubsection{Simple Spread}
%我们可以看到曲线，mager表现最好，尤其是到了50个智能体的时候，他很快速地收敛到了最优值，即接近100%成功。说明我们方法两阶段分配目标点和环境动作的优越性，可以快速到达目标点。反观其他baseline，mat在baseline中表现最好，在5agent也可快速收敛至最优值，可以推断出mat这种拿到前者智能体动作的条件动作输出还是可以更好地促进智能体之间的合作性。而随着智能体个数的增加，空间变大，mat的性能也急剧下降。在20agent是只能有80%左右，50agent只有10%+。最差的当属maser，虽然他是marl goal conditioned的方法，但他是value based，这种从reply buffer当中收集state再采集作为sub goal的方法十分不高效，对于多智能体环境中，学习不到最优值。
We demonstrate the training curves in Fig.~\ref{fig:baseline_sp} and the evaluation performance in \cref{tab: simple_spread}. The results suggest that {\name} performs the best, especially in scenarios with 50 agents, where it converges to the near-optimal solution quickly with a success rate of 100\%, attaining training efficiency more than $10\times$ higher than other competitors. The results show that our algorithm performs the best, especially in the scenario with 50 agents. This graph-enhanced hierarchical framework helps agents quickly handle the problem of reaching targets with high cooperation. MAT excels in other MARL baselines and can achieve a success rate of 100\% in the 5-agent setting, indicating that MAT agents profit from the action information of their teammates. However, as the number of agents increases, the performance of MAT degrades significantly. DiCG is on-par with MAPPO, which indicates that directly utilizing the graph-based method can't contribute to better cooperation and efficiency. Although MASER is also a goal-conditioned HRL method, it is the worst among all the competitors. It implies that the value-based method, MASER, fails to discover effective cooperation strategies within limited training steps since it infers subgoals from the experience replay buffer and lacks a strong connection between agents and target goals.



\input{AAMAS-2023 Formatting Instructions/table/simple_spread}
\input{AAMAS-2023 Formatting Instructions/table/push_ball}
\input{AAMAS-2023 Formatting Instructions/table/drone}
\subsubsection{Push Ball}
%我们是在5和20agent上做push ball的实验，push ball 比simple spread的难度加大，但是maser还是能获得几乎100%的成功率。反观其他baseline，在5agent的时候，除了mat，都陷入了near optimal的策略，平稳停留到20%左右的成功率，而mat虽然在20%成功率之后有上升，但也只是缓慢上升。更别提20agent了。maser仍然是最差的。实验结果，进一步说明了我们的算法在很难的任务上可以跳出因为选双重目标点而导致目标点分配不清晰，造成的局部最优问题。
As shown in Fig.~\ref{fig:baseline_pb} and \cref{tab: push_ball}, we conduct the experiments with $N\in\{20, 50\}$ agents in Push Ball. The difficulty of Push Ball lies in that it requires a two-stage goal assignment, i.e., the agents first get the designated ball and then reach the target landmark with the ball. Nevertheless, {\name} still achieves a 100\% success rate with few training timsteps. In contrast, except for MAT, whose success rate slightly increases, other baselines obtain suboptimal policies with a success rate of 20\% in the 5-agent setting. In the scenario with 20 agents, all baselines fail to reach the goals. The results express that the high-level Goal Commander in {\name} has the potential to simultaneously tackle multiple goal assignment problems, for it breaks this $M$\-stage goal assignment into $M$ independent tasks, only requiring the information of assigned targets.\looseness=-1
\subsubsection{Drones}
%无人机这个任务的结果再figure 7 和 表3，结果展示我们的方法依然还是最优的，在4agent的情况下，有快2倍的效率，成功率高10%和16%，在无人机中是mappo是次好的。可以看出在智能体数量较少的情况下，我们的算法优势减弱，但依然能是最好，而且在drone这种难度大的仿真环境中，我们也能到达90%和80%成功率，说明了之后在物理世界部署的可行性。
We report the training performance in Fig.~\ref{fig:baseline_drone} and the evaluation results in Fig.~\ref{fig:drone_inter} and \cref{tab: drone}. The experiment shows that {\name} is superior to other competitors with a success rate of 95\% in $N=2$ and 79\% in $N=4$ in the physically realistic 3D environment, Drone. Unlike MPE, the best competitor in Drone among baselines is MAPPO rather than MAT, indicating that MAPPO has better competence in complex tasks with few agents. Specifically, {\name} outperforms MAPPO, with 12\% higher and 15\% higher success rates in $N=2$ and $4$, respectively. Furthermore, {\name} manifests high coordination with a low collision rate of 0.02\% in $N=2$ and 0.12\% in $N=4$, demonstrating that {\name} succeeds in assigning target goals to agents to coordinate and capture the interaction among agents. Although MAPPO performs best among baselines, its collision rate is remarkably high. We speculate that MAPPO agent pursues high individual capability instead of cooperation. Furthermore, the sample efficiency of {\name} is $2\times$ higher than that of MAPPO in the 4-agent setting.


\subsection{Ablation Study}
To illustrate the effectiveness of each component of {\name}, we consider 3 variants of our method in Simple Spread with 50 agents:
\begin{itemize}
\setlength{\parskip}{0pt} 
\setlength{\itemsep}{0pt plus 1pt}
\item {\bf {\name} w. RG}: We substitute the Goal Scheduler in the Goal Commander with random sampling without replacement to assign each agent a random target goal.
\item {\bf \name-Atten}: We remove GCN in the Obs. Encoder and replace the Graph Encoder in the Action Executor with the attention module~\cite{ATTENTION} to extract the relationship of agents. The concatenation of $(f_o(o_1),f_o(o_2),..f_o(o_N))$ is fed into the attention module.
\item {\bf \name-MLP}: We consider the MLP layer as the alternative to the Action Executor to capture the correlation between agents and goals. The MLP layer takes the concatenation of $(f_o(o_1),f_o(o_2),..f_o(o_N), P_g)$ as input.
\end{itemize}

%ab的实验结果在fig和table里面，可以看出我们的方法还是最好，其中mlp的方法最差，说明单纯靠mlp参数太多，难以快速捕捉agent和goal的关系，没有分配权重。random goal表现也较差，因为没有一个上层好的分配点，有可能给智能体分配很远的goal，无法在有限时间步里使所有的agent都到达landmark。attn只是比我们的方法和gnn的主要区别在于，attn是对所有智能体都进行了权重分配，而我们的方法只提取了子图，只关注对我作用较大的智能体，故她不会被其他无用的智能体所干扰。所以
\begin{figure}
\captionsetup{justification=centering}
	\centering
 {\includegraphics[height=0.20\textwidth]{AAMAS-2023 Formatting Instructions/figures/ab.png}}
	\caption{\raggedright{Ablation study on {\name} in Simple Spread with $50$ agents.}}
\label{fig:ab}

\end{figure}

Fig.~\ref{fig:ab} and \cref{tab: ab} summarize the performance of {\name} and its variants on training and evaluation, respectively. {\name} excels in data efficiency and final performance with a 100\% success rate. \emph{{\name-MLP}} degrades most, implying that the MLP layer is incapable of distinguishing the correlation of agents and target goals from the given information. \emph{{{\name} w. RG}} lacks an appropriate Goal scheduler in the high-level Goal Commander, which may lead to agents being assigned distant goals. Therefore, {{\name} w. RG} reveals a worse performance with an 83\% success rate. \emph{{\name-Atten}} is slightly inferior to {\name} with a 7\% lower success rate. We hypothesize that \emph{{\name-Atten}} provides each agent with the attention weights of all the neighbors, where needless teammates may influence agents. On the contrary, {\name} agent only concentrates on crucial neighbors in the subgraph with useful information.\looseness=-1


%case study（todo）


==> AAMAS-2023 Formatting Instructions/6_conclusion.tex <==
\input{AAMAS-2023 Formatting Instructions/table/ab}
\section{Conclusion and Future Work}
In this paper, we propose a goal-conditioned MARL framework, \emph{Multi-Agent Commander-Executor}~(\name), to improve data efficiency and cooperation in multi-agent navigation tasks, especially in scenarios with large space spaces~(e.g., a massive number of agents or complex 3$D$ simulator). {\name} consists of a high-level Goal Commander and a low-level Action Executor, where the Commander allocates target goals to agents via the probability distribution of goals and the Executor leverages GNN and a Goal Encoder to capture team representation with strong goal guidance. Thorough experiments demonstrate that {\name} achieves higher sample efficiency and better performances than all the state-of-the-art MARL baselines in multi-agent particle environments~(MPE) with large-scale agents and a more complicated quadrotor navigation task. Currently, {\name} mainly focuses on multi-agent navigation tasks, and we will try to apply {\name} to other multi-agent tasks beyond navigation in the future. \looseness=-1



==> AAMAS-2023 Formatting Instructions/7_ac.tex <==
\section*{ACKNOWLEDGMENT}

This research was supported by National Natural Science Foundation of China (No.62203257, U19B2019, M-0248), Tsinghua University Initiative Scientific Research Program, Tsinghua-Meituan Joint Institute for Digital Life, Beijing National Research Center for Information Science, Technology (BNRist) and Beijing Innovation Center for Future Chips. 



==> table/ab.tex <==
% \usepackage{booktabs}

\begin{table}
\centering

\begin{tabular}{ccccc}
\toprule
             & \footnotesize{{\name} w. RG} & \footnotesize{\name-Atten} & \footnotesize{\name-MLP} & \footnotesize{\name}  \\ 
\midrule
Suc. Rate &    0.83\footnotesize{(0.01)}   &  0.93\footnotesize{(0.01)}     &   0.50\footnotesize{(0.08)}    &    {\bf1.00}\footnotesize{(0.01)}    \\

\bottomrule
\end{tabular}
\caption{ \raggedright{Evaluation performance of Success Rate between {\name} and its variants in Simple Spread.}}
\label{tab: ab}
\vspace{-9mm}
\end{table}
% \usepackage{booktabs}
% \bottomrule
% Steps &    0.83\footnotesize{(0.01)}   &       &   0.50\footnotesize{(0.08)}    &    1.00\footnotesize{(0.01)}    \\

==> table/drone.tex <==
% % \usepackage{booktabs}


% \begin{table}
% \centering

% \begin{tabular}{cc|c|c|c|c}
% \toprule
%              & MAPPO & MAT & DICG & MASER & MAGER  \\ 
% \midrule
% 2 agents &     0.83\footnotesize{(0.03)}  &   0.61\footnotesize{(0.01)}  &      &       &  0.95\footnotesize{(0.03)}       \\
% \midrule
% 4 agents &       &     &      &       &     0.83\footnotesize{(0.07)}   \\
% \bottomrule
% \end{tabular}
% \centering\caption{Evaluation performance of Success Rate between {\name} and baselines in Drones.}
% \label{tab: drone}
% \end{table}
% \usepackage{booktabs
% \usepackage{booktabs}

% \usepackage{booktabs}


\begin{table}
\centering
\begin{tabular}{ccc|cc}
\toprule
                     & \multicolumn{2}{c|}{2 agents}   & \multicolumn{2}{c}{4 agents}  \\ 
\cmidrule{2-5}  & Suc. Rate & Colli. Rate                                          & Suc. Rate & Colli. Rate       \\ 
\midrule
MAPPO             &          0.83\footnotesize{(0.03)}    &  0.10\footnotesize{(0.01)}&    0.64 \footnotesize{(0.01)}      &   0.18 \footnotesize{(0.02)}               \\ 
\midrule
MAT                 &   0.61\footnotesize{(0.01)}         &  0.09 \footnotesize{(0.01)}                                                      &    0.34\footnotesize{(0.04)}       &   {\bf0.06}\footnotesize{(0.01)}                \\ 
\midrule
DICG  &         0.45\footnotesize{(0.02)}      &     0.03\footnotesize{(0.02)}      & 0.12\footnotesize{(0.01)}&     0.07\footnotesize{(0.01) }                    \\ 
\midrule
{\name}                &          {\bf0.95}\footnotesize{(0.03)}  & {\bf0.02}\footnotesize{(0.01 )}                                            &      {\bf0.79}\footnotesize{(0.07)}        &  0.12   \footnotesize{(0.01)}                  \\
\bottomrule
\end{tabular}
\caption{ \raggedright{Evaluation performance of the success rate and the collision rate between {\name} and baselines in Drones.}}
\vspace{-5mm}
\label{tab: drone}
\end{table}


==> table/push_ball.tex <==
% \usepackage{booktabs}


\begin{table}
\centering

\begin{tabular}{cccccc}
\toprule
 & MAPPO & MAT & DICG & MASER & {\name}  \\ 
\midrule
5 agents&     0.20\footnotesize{(0.01)}&  0.32\footnotesize{(0.04)} &  0.20\footnotesize{(0.01)}&  0.01\footnotesize{(0.01)} & {\bf1.00}\footnotesize{(0.01)}        \\
\midrule
20 agents &    0.26\footnotesize{(0.01)}   &  0.25\footnotesize{(0.02)}   &   0.36\footnotesize{(0.01)}   &   0.01\footnotesize{(0.01)}    &     {\bf1.00}\footnotesize{(0.01)}    \\
\bottomrule
\end{tabular}
\caption{ \raggedright{Evaluation performance of the success rate between {\name} and baselines in Push Ball.}}
\vspace{-5mm}
\label{tab: push_ball}
\end{table}
% \usepackage{booktabs}


==> table/simple_spread.tex <==
% \usepackage{booktabs}


\begin{table}
\centering

\begin{tabular}{cccccc}
\toprule
  & MAPPO & MAT & DICG & MASER & {\name}  \\ 
\midrule
5 agents  &       0.82\footnotesize{(0.03)}& 1.00\footnotesize{(0.01)}    &  0.71\footnotesize{(0.05)}   &   0.06\footnotesize{(0.12)} & {\bf 1.00}\footnotesize{(0.01)}       \\
\midrule
20 agents &     0.50\footnotesize{(0.31)}  &    0.56\footnotesize{(0.26)} &   0.41\footnotesize{(0.04)}   &  0.02\footnotesize{(0.23)}     & {\bf 1.00}\footnotesize{(0.01)}       \\
\midrule
50 agents &       0.13\footnotesize{(0.02)} &     0.11\footnotesize{(0.01)}&  0.12\footnotesize{(0.02)}    &    0.01\footnotesize{(0.05)}   &    {\bf 1.00}\footnotesize{(0.01)}    \\

\bottomrule
\end{tabular}
\caption{ \raggedright{Evaluation performance of the success rate between {\name} and baselines in Simple Spread.}}
\vspace{-5mm}
\label{tab: simple_spread}
\end{table}
% \usepackage{booktabs}

==> table/simple_spread_all.tex <==
% \usepackage{booktabs}


\begin{table}
\centering

\begin{tabular}{cccc}
\toprule
 Agents & 5 &20 & 50  \\ 
\midrule
MA A*   &    {\bf 1.00}\footnotesize{(0.01)}& 0.93\footnotesize{(0.03)}  &   0.77\footnotesize{(0.03)}  \\
\midrule
{\name}  &     {\bf 1.00}\footnotesize{(0.01)}  &    {\bf 1.00}\footnotesize{(0.01)} &   {\bf 1.00}\footnotesize{(0.01)}\\ 

\bottomrule
\end{tabular}
\caption{ \raggedright{Evaluation performance of the success rate between {\name} and MA A$^*$ in Simple Spread.}}
\label{tab: simple_spread_all}
\end{table}
% \usepackage{booktabs}
